Space-time optimized table lookup

We describe a space-time optimized circuit for the table lookup subroutine from lattice-surgery surface code primitives respecting 2D grid connectivity. Table lookup circuits are ubiquitous in quantum computing, allowing the presented circuit to be used for applications ranging from cryptography to quantum chemistry. Surface code is the leading approach to scalable fault-tolerant quantum computing pursued by industry and academia. We abstract away surface code implementation details by using a minimal set of operations supported by the surface code via lattice-surgery. Our exposition is accessible to a reader not familiar with surface codes and fault-tolerant quantum computing.

==> circuits/layout/patch.tex <==
%auto-ignore
\begin{tikzpicture}[baseline=(base),x=.5cm,y=-.5cm]
\checkerboard{2}{2}
\fill[draw] (0,0) circle (2pt);
\coordinate (base) at (current bounding box.south);
\end{tikzpicture}


==> circuits/mini-measx.tex <==
%auto-ignore
\begin{tikzpicture}[x=.5cm,y=-.5cm,baseline=(base)]
    \checkerboard{2}{2}
    
    \begin{scope}[every node/.style={inner sep=1.5pt,font=\normalsize}]
    \node[shape=yquant-ft-measure,ft x] at (0,0) {X};
    \end{scope}
    
    \coordinate (base) at (current bounding box.center);
\end{tikzpicture}


==> circuits/mini-measz.tex <==
%auto-ignore
\begin{tikzpicture}[x=.5cm,y=-.5cm,baseline=(base)]
    \checkerboard{2}{2}
    
    \begin{scope}[every node/.style={inner sep=1.5pt,font=\normalsize}]
    \node[shape=yquant-ft-measure,ft z] at (0,0) {\zonx};
    \end{scope}
    
    \coordinate (base) at (current bounding box.center);
\end{tikzpicture}


==> circuits/mini-prepx.tex <==
%auto-ignore
\begin{tikzpicture}[x=.5cm,y=-.5cm,baseline=(base)]
    \checkerboard{2}{2}
    
    \begin{scope}[every node/.style={inner sep=1.5pt,font=\normalsize}]
    \node[shape=yquant-ft-prepare,ft x] at (0,0) {X};
    \end{scope}
    
    \coordinate (base) at (current bounding box.center);
\end{tikzpicture}


==> circuits/mini-prepz.tex <==
%auto-ignore
\begin{tikzpicture}[x=.5cm,y=-.5cm,baseline=(base)]
    \checkerboard{2}{2}
    
    \begin{scope}[every node/.style={inner sep=1.5pt,font=\normalsize}]
    \node[shape=yquant-ft-prepare,ft z] at (0,0) {\zonx};
    \end{scope}
    
    \coordinate (base) at (current bounding box.center);
\end{tikzpicture}


==> circuits/mt-cnot-2.tex <==
%auto-ignore
\begin{tikzpicture}[x=.5cm,y=-.5cm,baseline=(base)]
    \checkerboard{5}{2}
    
    \coordinate (c1) at (0,1);
    \coordinate (c2) at (0,4);
    
    \ZCatCoord{c1}{c2}

    \coordinate (base) at (current bounding box.center);
\end{tikzpicture}

